Flexible domain prediction using mixed effects random forests

This paper promotes the use of random forests as versatile tools for estimating spatially disaggregated indicators in the presence of small area-specific sample sizes. Small area estimators are predominantly conceptualized within the regression-setting and rely on linear mixed models to account for the hierarchical structure of the survey data. In contrast, machine learning methods offer non-linear and non-parametric alternatives, combining excellent predictive performance and a reduced risk of model-misspecification. Mixed effects random forests combine advantages of regression forests with the ability to model hierarchical dependencies. This paper provides a coherent framework based on mixed effects random forests for estimating small area averages and proposes a non-parametric bootstrap estimator for assessing the uncertainty of the estimates. We illustrate advantages of our proposed methodology using Mexican income-data from the state Nuevo Le\'on. Finally, the methodology is evaluated in model-based and design-based simulations comparing the proposed methodology to traditional regression-based approaches for estimating small area averages.

==> Submitted Version arxiv/Tables/table_DB.tex <==


\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates including details on in- and out-of-sample areas} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
		\\[-1.8ex]\hline 
		\hline \\[-1.8ex] 
		& &\multicolumn{2}{c}{Total} &\multicolumn{2}{c}{In-sample}&\multicolumn{2}{c}{Out-of-sample} \\
		\hline \\[-1.8ex]
		& & Median & Mean & Median & Mean & Median & Mean \\ 
		\hline \\[-1.8ex] 
		\multirow{ 4}{*}{RB}
		&BHF & $0.142$ & $0.178$ & $0.051$ & $0.112$ & $0.218$ & $0.224$ \\ 
		&EBP & $0.147$ & $0.179$ & $0.053$ & $0.117$ & $0.226$ & $0.223$ \\			 
		&EBP-BC & $0.096$ & $0.184$ & $0.061$ & $0.072$ & $0.158$ & $0.263$ \\			 
		&MERF & $0.077$ & $0.186$ & $0.035$ & $0.172$ & $0.106$ & $0.196$ \\
		\hline \\[-1.8ex] 
		\multirow{ 4}{*}{RRMSE}
		&BHF & $0.149$ & $0.216$ & $0.095$ & $0.170$ & $0.230$ & $0.248$ \\
		&EBP & $0.159$ & $0.217$ & $0.095$ & $0.174$ & $0.229$ & $0.247$ \\ 
		&EBP-BC & $0.140$ & $0.239$ & $0.129$ & $0.152$ & $0.161$ & $0.299$ \\ 
		&MERF  & $0.094$ & $0.212$ & $0.061$ & $0.199$ & $0.125$ & $0.221$ \\			
		\hline \\[-1.8ex] 
	\end{tabular}
\end{table}



==> Submitted Version arxiv/Tables/table_MB.tex <==
\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates in 4 settings} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
		\\[-1.8ex]\hline 
		\hline \\[-1.8ex] 
		& &\multicolumn{2}{c}{\textit{Normal}} &\multicolumn{2}{c}{\textit{Interaction}}&\multicolumn{2}{c}{\textit{Normal-Par}}&\multicolumn{2}{c}{\textit{Interaction-Par}} \\
		\hline \\[-1.8ex]
		& & Median & Mean & Median & Mean & Median & Mean & Median & Mean \\ 
		\hline \\[-1.8ex] 
		\multirow{ 4}{*}{RB}
		&BHF & $0.001$ & $0.001$ & $$-$0.002$ & $0.001$ & $0.002$ & $0.002$ & $0.000$ & $0.001$ \\ 
		&EBP & $0.001$ & $0.001$ & $$-$0.001$ & $0.001$ & $0.002$ & $0.002$ & $0.001$ & $0.001$ \\ 
		&EBP-BC & $0.002$ & $0.002$ & $0.002$ & $0.004$ & $0.002$ & $0.001$ & $0.001$ & $0.003$ \\
		&MERF & $0.001$ & $0.002$ & $0.003$ & $0.003$ & $0.004$ & $0.004$ & $0.002$ & $0.002$ \\
		\hline \\[-1.8ex]
		\multirow{ 4}{*}{RRMSE} 
		&BHF & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\ 
		&EBP & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\
		&EBP-BC & $0.040$ & $0.042$ & $0.036$ & $0.038$ & $0.035$ & $0.038$ & $0.027$ & $0.028$ \\  
		&MERF & $0.042$ & $0.045$ & $0.023$ & $0.024$ & $0.039$ & $0.044$ & $0.014$ & $0.015$ \\ 
		\hline \\[-1.8ex] 
	\end{tabular}
\end{table}

==> Submitted Version arxiv/Tables/tablesBackup_column.tex <==
\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates in 4 settings} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
			\\[-1.8ex]\hline 
			\hline \\[-1.8ex] 
			& &\multicolumn{2}{c}{\textit{Normal}} &\multicolumn{2}{c}{\textit{Interaction}}&\multicolumn{2}{c}{\textit{Normal-Par}}&\multicolumn{2}{c}{\textit{Interaction-Par}} \\
			\hline \\[-1.8ex]
			& & Median & Mean & Median & Mean & Median & Mean & Median & Mean \\ 
			\hline \\[-1.8ex] 
			\multicolumn{9}{l}{RB}\\
			\hline \\[-1.8ex]
			&BHF & $0.001$ & $0.001$ & $$-$0.002$ & $0.001$ & $0.002$ & $0.002$ & $0.000$ & $0.001$ \\ 
			&EBP & $0.001$ & $0.001$ & $$-$0.001$ & $0.001$ & $0.002$ & $0.002$ & $0.001$ & $0.001$ \\ 
		 	&EBP-BC & $0.002$ & $0.002$ & $0.002$ & $0.004$ & $0.002$ & $0.001$ & $0.001$ & $0.003$ \\
		 	&MERF & $0.001$ & $0.002$ & $0.003$ & $0.003$ & $0.004$ & $0.004$ & $0.002$ & $0.002$ \\
		 	\hline \\[-1.8ex]
		 	\multicolumn{9}{l}{RRMSE}\\
		 	\hline \\[-1.8ex] 
			&BHF & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\ 
			&EBP & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\
			&EBP-BC & $0.040$ & $0.042$ & $0.036$ & $0.038$ & $0.035$ & $0.038$ & $0.027$ & $0.028$ \\  
			&MERF & $0.042$ & $0.045$ & $0.023$ & $0.024$ & $0.039$ & $0.044$ & $0.014$ & $0.015$ \\ 
			\hline \\[-1.8ex] 
	\end{tabular}
\end{table} 

\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates including details on in- and out-of-sample areas} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
		\\[-1.8ex]\hline 
		\hline \\[-1.8ex] 
		& &\multicolumn{2}{c}{Total} &\multicolumn{2}{c}{In-sample}&\multicolumn{2}{c}{Out-of-sample} \\
		\hline \\[-1.8ex]
		& & Median & Mean & Median & Mean & Median & Mean \\ 
		\hline \\[-1.8ex] 
		\multicolumn{7}{l}{RB}\\
		\hline \\[-1.8ex]
		&BHF & $0.142$ & $0.178$ & $0.051$ & $0.112$ & $0.218$ & $0.224$ \\ 
		&EBP & $0.147$ & $0.179$ & $0.053$ & $0.117$ & $0.226$ & $0.223$ \\			 
		&EBP-BC & $0.096$ & $0.184$ & $0.061$ & $0.072$ & $0.158$ & $0.263$ \\			 
		&MERF & $0.077$ & $0.186$ & $0.035$ & $0.172$ & $0.106$ & $0.196$ \\
		\hline \\[-1.8ex] 
		\multicolumn{7}{l}{RRMSE}\\
		\hline \\[-1.8ex]
		&BHF & $0.149$ & $0.216$ & $0.095$ & $0.170$ & $0.230$ & $0.248$ \\
		&EBP & $0.159$ & $0.217$ & $0.095$ & $0.174$ & $0.229$ & $0.247$ \\ 
		&EBP-BC & $0.140$ & $0.239$ & $0.129$ & $0.152$ & $0.161$ & $0.299$ \\ 
		&MERF  & $0.094$ & $0.212$ & $0.061$ & $0.199$ & $0.125$ & $0.221$ \\			
		\hline \\[-1.8ex] 
	\end{tabular}
\end{table}

==> Tables/table_DB.tex <==


\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates including details on in- and out-of-sample areas} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
		\\[-1.8ex]\hline 
		\hline \\[-1.8ex] 
		& &\multicolumn{2}{c}{Total} &\multicolumn{2}{c}{In-sample}&\multicolumn{2}{c}{Out-of-sample} \\
		\hline \\[-1.8ex]
		& & Median & Mean & Median & Mean & Median & Mean \\ 
		\hline \\[-1.8ex] 
		\multirow{ 4}{*}{RB}
		&BHF & $0.142$ & $0.178$ & $0.051$ & $0.112$ & $0.218$ & $0.224$ \\ 
		&EBP & $0.147$ & $0.179$ & $0.053$ & $0.117$ & $0.226$ & $0.223$ \\			 
		&EBP-BC & $0.096$ & $0.184$ & $0.061$ & $0.072$ & $0.158$ & $0.263$ \\			 
		&MERF & $0.077$ & $0.186$ & $0.035$ & $0.172$ & $0.106$ & $0.196$ \\
		\hline \\[-1.8ex] 
		\multirow{ 4}{*}{RRMSE}
		&BHF & $0.149$ & $0.216$ & $0.095$ & $0.170$ & $0.230$ & $0.248$ \\
		&EBP & $0.159$ & $0.217$ & $0.095$ & $0.174$ & $0.229$ & $0.247$ \\ 
		&EBP-BC & $0.140$ & $0.239$ & $0.129$ & $0.152$ & $0.161$ & $0.299$ \\ 
		&MERF  & $0.094$ & $0.212$ & $0.061$ & $0.199$ & $0.125$ & $0.221$ \\			
		\hline \\[-1.8ex] 
	\end{tabular}
\end{table}



==> Tables/table_MB.tex <==
\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates in 4 settings} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
		\\[-1.8ex]\hline 
		\hline \\[-1.8ex] 
		& &\multicolumn{2}{c}{\textit{Normal}} &\multicolumn{2}{c}{\textit{Interaction}}&\multicolumn{2}{c}{\textit{Normal-Par}}&\multicolumn{2}{c}{\textit{Interaction-Par}} \\
		\hline \\[-1.8ex]
		& & Median & Mean & Median & Mean & Median & Mean & Median & Mean \\ 
		\hline \\[-1.8ex] 
		\multirow{ 4}{*}{RB}
		&BHF & $0.001$ & $0.001$ & $$-$0.002$ & $0.001$ & $0.002$ & $0.002$ & $0.000$ & $0.001$ \\ 
		&EBP & $0.001$ & $0.001$ & $$-$0.001$ & $0.001$ & $0.002$ & $0.002$ & $0.001$ & $0.001$ \\ 
		&EBP-BC & $0.002$ & $0.002$ & $0.002$ & $0.004$ & $0.002$ & $0.001$ & $0.001$ & $0.003$ \\
		&MERF & $0.001$ & $0.002$ & $0.003$ & $0.003$ & $0.004$ & $0.004$ & $0.002$ & $0.002$ \\
		\hline \\[-1.8ex]
		\multirow{ 4}{*}{RRMSE} 
		&BHF & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\ 
		&EBP & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\
		&EBP-BC & $0.040$ & $0.042$ & $0.036$ & $0.038$ & $0.035$ & $0.038$ & $0.027$ & $0.028$ \\  
		&MERF & $0.042$ & $0.045$ & $0.023$ & $0.024$ & $0.039$ & $0.044$ & $0.014$ & $0.015$ \\ 
		\hline \\[-1.8ex] 
	\end{tabular}
\end{table}

==> Tables/tablesBackup_column.tex <==
\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates in 4 settings} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
			\\[-1.8ex]\hline 
			\hline \\[-1.8ex] 
			& &\multicolumn{2}{c}{\textit{Normal}} &\multicolumn{2}{c}{\textit{Interaction}}&\multicolumn{2}{c}{\textit{Normal-Par}}&\multicolumn{2}{c}{\textit{Interaction-Par}} \\
			\hline \\[-1.8ex]
			& & Median & Mean & Median & Mean & Median & Mean & Median & Mean \\ 
			\hline \\[-1.8ex] 
			\multicolumn{9}{l}{RB}\\
			\hline \\[-1.8ex]
			&BHF & $0.001$ & $0.001$ & $$-$0.002$ & $0.001$ & $0.002$ & $0.002$ & $0.000$ & $0.001$ \\ 
			&EBP & $0.001$ & $0.001$ & $$-$0.001$ & $0.001$ & $0.002$ & $0.002$ & $0.001$ & $0.001$ \\ 
		 	&EBP-BC & $0.002$ & $0.002$ & $0.002$ & $0.004$ & $0.002$ & $0.001$ & $0.001$ & $0.003$ \\
		 	&MERF & $0.001$ & $0.002$ & $0.003$ & $0.003$ & $0.004$ & $0.004$ & $0.002$ & $0.002$ \\
		 	\hline \\[-1.8ex]
		 	\multicolumn{9}{l}{RRMSE}\\
		 	\hline \\[-1.8ex] 
			&BHF & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\ 
			&EBP & $0.039$ & $0.042$ & $0.037$ & $0.039$ & $0.037$ & $0.042$ & $0.028$ & $0.030$ \\
			&EBP-BC & $0.040$ & $0.042$ & $0.036$ & $0.038$ & $0.035$ & $0.038$ & $0.027$ & $0.028$ \\  
			&MERF & $0.042$ & $0.045$ & $0.023$ & $0.024$ & $0.039$ & $0.044$ & $0.014$ & $0.015$ \\ 
			\hline \\[-1.8ex] 
	\end{tabular}
\end{table} 

\begin{table}[!h] 
	\centering
	\captionsetup{justification=centering,margin=1.5cm} 
	\caption{Mean and Median of RB and RRMSE for point-estimates including details on in- and out-of-sample areas} 
	\label{} 
	\begin{tabular}{@{\extracolsep{5pt}} lrcccccccc} 
		\\[-1.8ex]\hline 
		\hline \\[-1.8ex] 
		& &\multicolumn{2}{c}{Total} &\multicolumn{2}{c}{In-sample}&\multicolumn{2}{c}{Out-of-sample} \\
		\hline \\[-1.8ex]
		& & Median & Mean & Median & Mean & Median & Mean \\ 
		\hline \\[-1.8ex] 
		\multicolumn{7}{l}{RB}\\
		\hline \\[-1.8ex]
		&BHF & $0.142$ & $0.178$ & $0.051$ & $0.112$ & $0.218$ & $0.224$ \\ 
		&EBP & $0.147$ & $0.179$ & $0.053$ & $0.117$ & $0.226$ & $0.223$ \\			 
		&EBP-BC & $0.096$ & $0.184$ & $0.061$ & $0.072$ & $0.158$ & $0.263$ \\			 
		&MERF & $0.077$ & $0.186$ & $0.035$ & $0.172$ & $0.106$ & $0.196$ \\
		\hline \\[-1.8ex] 
		\multicolumn{7}{l}{RRMSE}\\
		\hline \\[-1.8ex]
		&BHF & $0.149$ & $0.216$ & $0.095$ & $0.170$ & $0.230$ & $0.248$ \\
		&EBP & $0.159$ & $0.217$ & $0.095$ & $0.174$ & $0.229$ & $0.247$ \\ 
		&EBP-BC & $0.140$ & $0.239$ & $0.129$ & $0.152$ & $0.161$ & $0.299$ \\ 
		&MERF  & $0.094$ & $0.212$ & $0.061$ & $0.199$ & $0.125$ & $0.221$ \\			
		\hline \\[-1.8ex] 
	\end{tabular}
\end{table}
